cISP: A Speed-of-Light Internet Service Provider

Low latency is a requirement for a variety of interactive network applications. The Internet, however, is not optimized for latency. We thus explore the design of cost-effective wide-area networks that move data over paths very close to great-circle paths, at speeds very close to the speed of light in vacuum. Our cISP design augments the Internet's fiber with free-space wireless connectivity. cISP addresses the fundamental challenge of simultaneously providing low latency and scalable bandwidth, while accounting for numerous practical factors ranging from transmission tower availability to packet queuing. We show that instantiations of cISP across the contiguous United States and Europe would achieve mean latencies within 5% of that achievable using great-circle paths at the speed of light, over medium and long distances. Further, we estimate that the economic value from such networks would substantially exceed their expense.

==> discussion.tex <==
  

\section{Discussion}
\label{sec:discussion}

Designing an ISP under the constraints imposed by microwave radios poses several challenges, and may even seem unrealistic at first glance. However, our results and analysis demonstrate that building a wide-area network that operates nearly at the speed of light in vacuum, is not only practically feasible, but also surprisingly cost-effective, and provides significant application-layer performance improvements. Many years of operational experience with long-distance links used in the HFT industry set the stage for this work, and provide assurance about the feasibility of our proposal. In the following we attempt to address some of the concerns this work may raise.

\paragraphb{Isn't Microwave so 1960s?} AT\&T had a rich MW deployment for radio and TV signals as far back as 1960~\cite{attLongLines}. Over long distances, such communication has steadily moved towards fiber. However, four key developments make our MW-based proposal attractive today: (a) New applications unthought of in the pre-Internet era have made low latency extremely valuable. (b) The High Frequency Trading (HFT) race for connecting Chicago-New York Stock exchanges has, over the past few years, led to the development of MW radios that function at much lower latencies, adding a negligible few $\mu s$ per hop. This recent advance is crucial to the application of MW for low latency. (c) Advances in geographical information systems and automated route planning have dramatically improved deployment efficiency,routing latencies, and costs relative to the ``hand planned'' MW links of 1960s. (d) We demonstrate that the limited bandwidth can be exploited meaningfully to benefit application performance.

\paragraphb{Wireless-only or hybrid?} While our results demonstrate that even the limited capacity of microwave based networks can be used to benefit applications, we are also exploring a hybrid network, combining fiber and wireless links in parallel, whereby certain high-utilization wireless segments could fall back some traffic to fiber. Further, as of now, no suitable wireless solution has bridged the continental divide. However, decreasing intra-continental latency itself would be highly valuable.
%This may pose new challenges, such as increasing the variation in RTTs depending on whether packets are sent over wireless or fiber links.

\paragraphb{Impact of weather:} Microwave transmissions are attenuated by both rainfall and humidity. 
%The method and fitting formulae of ITU-R P 853-3~\cite{weather} constitute a generally accepted procedure for estimating link attenuation in dB/km as a function of frequency and the local rainfal rate, whereas the methodology of ITU-R P 676-9~\cite{gases} is generally used to compute atmospheric attenuation as a function of frequency, humidity and temperature. 
Based on standards for measuring atmospheric attenuation~\cite{gases} and rainfall-induced attenuation~\cite{weather}, Laughlin et al.~\cite{cost} estimated microwave links used in this work to have $99\%$+ availability at $256$ QAM modulation using standard FCC-approved radio TX power settings. Further, when certain segments are unavailable, falling back to fiber for those segments will still provide latency improvements from other segments on the path, thus gracefully degrading the latency improvement cISP achieves.
%We will have lower layer mechanisms to ensure reliability.

\paragraphb{Connecting to cISP:} We presented results on the operation of cISP and its benefits, without addressing how users and other networks would connect to this network. Users connecting directly could use a VPN-like client installed on their devices, which would allow them to connect to their closest cISP location, tunneling their traffic as close to their destination as possible. Other ISPs and Web service providers could connect to cISP at Internet exchanges and colocation centers. cISP would, in fact, encourage hot-potato routing to provide the maximum possible latency improvements.

%Since we focus on 120 cities and data centers, these edge towers will be close to a co-location center in one of these cities or near a data center. We would like to build peering relationships with various content providers and other ISPs. Drawing insights from previous measurement studies, we expect that the additional cost for companies like Google, Amazon, Facebook etc. will be trivial compared to their boost in revenue. This would also be beneficial to ISPs since they can hand-over user traffic sooner, burning less resources in their network. We, in fact, would encourage hot potato routing by ISPs to improve performance of their customers!

%While the bandwidth of MW radios is improving, it is still far lower than fiber. Aggregate throughput supported by microwave-based cISP is also much lower than traditional ISPs. However, we intend to focus on low bandwidth applications such as web browsing initially. For gaming applications, our network will cater to low bandwidth control messages, i.e., communication in one direction only. As we saw in the experiments, even optimized latency in one direction can reduce frame time significantly. 

%We also plan to develop a hybrid network -- with wireless and fiber links in parallel -- in the wide area. This will combine best of both worlds - providing low latency as well as high bandwidth. However, this direction requires further exploration, particularly for TCP flows that estimate RTT to make control decisions. Alternating between the two networks could will lead to wide variations in RTT. However, this network will allow us to support both forward and reverse communication paths of the gaming application on the same network as long as they stick to the same network in a given direction. Fiber links can also serve as a fallback during wireless outages.

\paragraphb{Alternative low-latency technologies:} Due to the relatively low bandwidth of microwave, the search for alternative low-latency medium is active, with several new technologies having been proposed recently. This includes a millimeter wave-FSO hybrid which is commercialized, as well as hollow-core optical fiber by DARPA~\cite{hollowFiber} and millimeter-wave on power lines (AirGig by AT\&T~\cite{airGig}) which are currently in the research phase. Recently, Connectivity lab at Facebook succeeded in transmitting $20$~Gbps over $13$~km at speed-of-light using millimeter waves alone~\cite{fbMm}. This is $20\times$ higher than $1$~Gbps bandwidth of microwave links. These advances can only improve the cost-benefit compared to the design presented here, which is general enough to use any underlying technology.



%However, this work proposes that we \emph{augment} the strength of present fiber infrastructure (high bandwidth) with that of MW (low latency), using its limited capacity to carefully speed up only the latency-sensitive traffic (\S\ref{sec:webeval}). Without such an approach, long-distance MW-networks would perhaps remain limited to niches like HFT.



==> exp-methodology.tex <==
\section{Experimental results}
\label{sec:exp-methodology}

We experimentally show that a nearly speed-of-light Internet Service
Provider can be built in a cost-effective manner with minimal
extensions to existing infrastructure. We elaborate on the methodology
before delving into the results.

\subsection{Methodology}
In this section, we present our methodology and a detailed description
of the components used in the underlying infrastructure.

Microwave network design is based on tower information in the
continental United States obtained from ~\cite{fccasr}. 
We use a maximum link distance of $100$km and visibility constraints based on top-of-the tower height. We rely on (commercially available) microwave antennas to
compute the cost and bandwidth.

We use the network simulator ns-3\cite{ns3} for packet-level
simulations. We use UDP traffic with a uniform packet size of 500 bytes.
The built-in FlowMonitor\cite{flowMonitor} is used to measure delay
and loss rate. A new monitoring module is added to track link-level
utilization. Since the default routing in ns-3 was hop-based shortest
path routing, static routing with multiple weighted next-hops was
implemented to compare various routing schemes. All experiments simulate
$100Gbps$ of network traffic for $1$s of simulated time.  An
experiment takes approximately $10-12$ hours to complete on a single
core of a $3.1$GHz processor.

%\begin{figure}
%\centering
%\includegraphics[width=3.3in]{figures/user-GoogleDC-100Gbps.png}
%%\vspace{-6pt}
%\caption{\small \em }
%\label{fig:map1}
%\end{figure}

\paragraphb{Traffic classes:}
The traffic in cISP can be broadly classified into 3 categories. 

\textit{User-User: } This category comprises of traffic between users that
does not traverse a data center/cloud. This includes
interactive applications and other user-user flows. We focus on users
in 120 population centers, which covers \textasciitilde85\% of the US
population.   The weight associated with a city $i$ is given by its
population $p_i$. A flow between cities $i$ and $j$ has a weight of
$p_i * p_j$.

\textit{Data Center-Data Center (DC-DC):} We use Google data centers
as an example for building a low latency network connecting data
centers. We consider all the 6 publicly available Google data center
locations - Berkeley, SC; Council Bluffs, IA; Douglas County, GA;
Lenoir, NC; Mayes County, OK; and Dallas, OR. Since the
characteristics of low-latency traffic between data centers is not
available, we provision equal capacity between all pairs of data
centers.  All flows are assigned a weight of $1$.

\textit{User-Data Center (User-DC):} Each of the 120 cities is assumed
to send traffic to the closest Google DC. This traffic is weighted by
the population of the city, $p_i$.

Initially, we study each of the traffic classes separately to
understand their characteristics.   The user-user traffic class/network is
chosen as a representative when the classes have similar performance
for a metric.  Finally, we present results on the performance of a combined
network that connects all cities and data centers and handles all
classes of traffic.




==> fiberDesign.tex <==
\section{Making the most of fiber}
\label{sec:fiberDesign}

Present day Internet infrastructure comprises hundreds of thousands of miles of fiber optic cables. It is thus natural to ask: how close to speed of light latencies could we get using all the available fiber, unencumbered by economics driven ISP constraints on routing?

%\paragraphb{Fiber Dataset:} 
Recently Durairajan et al. analyzed US fiber 
infrastructure~\cite{intertubes} compiling various public sources of information. 
%Utilizing published 
%network maps of large ISPs, publicly available government records, contractual agreements, etc.
%the authors compiled and published a map of the long-haul fiber optic links in contiguous USA.
Their published dataset includes $540$ long-haul links between $273$ endpoints. We base our design and analysis on this dataset; we do not believe that any small inaccuracies will change our main conclusions. Additional fiber links that may be missing here would only improve this network's potential latency performance.
%Our analysis in this section, and the 
%network we design is based on this dataset.

We compute the shortest fiber paths between all pairs of endpoints in this dataset, and compare it to the geodesic distance between each pair of end points, yielding us a measure of stretch\footnote{All stretch values reported in this section take the speed-of-light in fiber into account, which is roughly $2/3$ of speed-of-light in vacuum.}. 
The median and $95$-th percentile stretch are $1.93$ and $2.72$ respectively. These values reflect the achievable 
inflation beyond $c$-latency on a network using all available (known) fiber in the US, assuming each fiber end-point 
contributes equally to the traffic. When a gravity model of traffic is used (\ie traffic between two locations is 
proportional to the product of their populations), the median and $95$-th percentile values are $1.85$ and $2.29$. 

%To evaluate the potential of this dataset for architecting a low-latency network, we computed the shortest paths 
%between all pairs of endpoints in this dataset and computed the ratio of the shortest 
%path length to the geodesic distance between each pair (i.e., stretch). The results are promising, as the median 
%stretch is found as $1.93$ and $95$-th percentile stretch is found as $2.72$. When 
%we use the gravity model (meaning the traffic between two locations is assumed to be proportional to the product of 
%their populations) the results are even better, with median and $95$-th percentile values $1.87$ and $2.42$. 

\begin{table}[]
\centering
\begin{tabular}{lll}
ISP & Median & 95th. prc. \\
\hline
EarthLink 	&1.98 & 2.68  \\
Level3 		& 1.99 & 2.68  \\
Comcast 	& 2.17 & 3.09  \\
CenturyLink 	& 2.27 & 4.94  \\
TWC 		& 2.17 & 2.98  \\
Verizon 	& 2.26 & 3.17 \\
ATT 		& 2.10 & 3.90 \\
Sprint		& 2.56 & 8.02 \\
HE		& 2.13 & 3.91
\end{tabular}
\caption{Stretch values for all pairs shortest paths}
\label{table-isp-size}
\end{table}

Further, Table~\ref{table-isp-size} also shows the median and $95$-th percentile stretch values for the $9$ largest ISPs, each of which has
long-haul links connecting over $100$ locations. The median stretch across these networks is smaller than that reported 
in earlier work~\cite{soslow-pam17} analyzing research networks such as Internet2. Note that the values in 
Table~\ref{table-isp-size} are not directly comparable to the stretch values we compute above for the entire set of 
$273$ locations -- no single ISP covers all locations, with the largest covering $248$ -- but even when covering fewer 
locations, individual ISP networks show higher stretch. Further, a recent measurement study~\cite{soslow-pam17} has 
reported end-to-end latencies over default routes between well-connected locations as $3$-$4\times$ inflated over 
$c$-latency. Thus, being able to aggregate and utilize the entirety of this fiber infrastructure could reduce latencies 
by as much as $50\%$. In the following, we estimate the performance and cost of such a network connecting large 
population centers.

%Though the stretch values are promising, they are significantly lower compared to values that was reported 
%before for other networks~\cite{soslow-pam17}. The median stretch is reported as $2.6$, $2.7$ and $3.6$ for Internet2, 
%ESnet, and GEANT respectively. One reason for a better stretch value for the current fiber map might be that it is a 
%superset of the links of 19 different ISPs and the results for individual ISPs would be closer to the previously 
%observed values. 
%Table~\ref{table-isp-size} shows the median and $95$-th percentile stretch values for the $9$ largest ISPs which have 
%long-haul links in over 100 locations in the InterTubes dataset.\footnote{Based on the reported link ownership/sharing 
%information in the InterTubes dataset, which might not cover all long-haul links of all the ISPs.} The stretch 
%values are indeed higher compared to 
%the entire dataset, and closer to the previously observed values. The low stretch value for the published dataset is 
%achieved since links from different ISPs are aggregated.

\paragraphb{Network design:} We use the $120$ largest population centers in the US as our network's end-points.
The mean distance 
between these population centers and their corresponding nearest fiber conduit endpoints in the 
fiber map is small ($5.1$~km), so we use these nearby fiber endpoints and our population centers interchangeably. We find that a fiber network using all the edges on the shortest paths between all pairs of target endpoints uses $348$ links, and $137,500$ km of fiber, and achieves a weighted median stretch of $1.87$.

%Even though it is desirable, it is not feasible to connect all target locations with shortest paths.
To investigate the impact of using a subset of these edges instead of all, we prune links that impact stretch minimally using an iterative heuristic: 
at each step, of all links not essential to maintaining connectivity are tested, and the link which causes the minimum increase in the mean stretch is removed.

% There are two reasons for going with this simple algorithm for the fiber network. First, we 
% start with almost $2 \times$ inflation over line-of-sight distances in the median, it makes sense to optimize only for 
% stretch and to always use the shortest paths in the fiber network. Second, bandwidth over fiber is virtually unlimited 
% compared to microwave links. Hence, even though some links might require significantly more capacity than others, 
% the bandwidth requirements are easier to satisfy.

Fig.~\ref{fig:fiber-cost-stretch} shows the mean, median, and $95$-th percentile stretch for networks built with different numbers of fiber edges.
Stretch does not change appreciably until a large number of links are discarded (leftward on the $x$-axis). 
One example network with $268$ links between $190$ locations with $82,000$ km of fiber is shown in Fig.~\ref{fig:fiber-design}.
%The increase in stretch until we remove around $80$ links is not very high, but beyond that 
%stretch values start to increase further. Figure~\ref{fig:fiber-design} shows the generated topology with $268$ links 
%between $190$ locations with $82,000$ km of fiber. 
The median, mean and $95$-th percentile stretch values for this 
network are $1.88$, $1.96$ and $2.77$ respectively, and in terms of network hops, the average path length between two population centers 
is $9$. Thicker lines and darker shades show higher utilization under shortest path routing. Note that while the dataset includes actual
fiber lengths, the map only draws geodesics between link end points.
%Our dataset only includes location of link endpoints and link lengths, so in the figure each link is 
%drawn as a straight line connecting the endpoints. We discuss our cost estimation of building this network next. 
 


\begin{figure}
\centering
\includegraphics[width=3.2in]{figures/nlinks_cost_vs_stretch.pdf}
\caption{The trade-off between the number of links in the fiber network topology, stretch and cost of the 
network}
\label{fig:fiber-cost-stretch}
\end{figure}

\begin{figure*}
\centering
\includegraphics[width=6.4in]{figures/fiberDesign}
\caption{The fiber network which connects the $120$ population centers with $268$ links and $82,000$km of fiber.
Increasing link capacities along the heavy traffic routes are marked with darker colors and thicker lines.}
\label{fig:fiber-design}
\end{figure*}

\paragraphb{Cost estimation:} What would it cost to be able to use fiber across service providers in this way? 
We use a $1$Tbps aggregate input rate to address this question, but arrive at a per unit bandwidth estimate that does not change substantially with aggregate input rate.
Our cost analysis is based on leasing the necessary fiber links, specifically, using short term -- $3$-$5$ years in this context -- wavelength leases.
Typically, wavelength services are available at $1$, $10$, $40$ and, $100$ Gbps, and prices vary 
depending on bandwidth, distance, route, carrier, and contract length. For a few key routes such as New York to Los Angeles, and, New York to
Chicago, we found pricing for $10$ and $100$ Gbps wavelengths in the form of $\$ / (\text{Gbps} * \text{km})/\text{month}$~\cite{100G-price,pricingTrends}. For 
example, the median $100$G wavelength price for the New York - Chicago is $\sim$$\$30,000$ per month, and the distance 
is ~$1,200$ km, computing to roughly ~$0.25$ $\$ / (\text{Gbps} * \text{km})/\text{month}$. This price 
estimate is for a $5$ year contract. For each site, we estimate an equipment cost of $\$10,000$ and a monthly 
colocation fee of $\$2,000$. 

%There are two ways of leasing fiber: lease dark fiber by signing an IRU 
%(Indefeasible Right of Use), typically for 20 years, or buy wavelengths over target links according to bandwidth 
%requirements. 
%
%The advantages of dark fiber include 
%complete control over the links and equipment, which can be upgraded at will to meet increasing bandwidth requirements 
%without need to renegotiate contracts. Moreover, with specialized transmission equipment it is possible to reduce 
%additional latency per hop. However, dark fiber leases with IRUs 
%require payment of a large sum upfront in addition to the cost of equipment to light the fiber. For example, assuming 
%$\$1,500$ per mile per strand as an average lease price (estimate based on the prices given in the 
%report~\cite{darkFiber}), the network in 
%figure~\ref{fig:fiber-design} will require $\$240,000,000$ just for the upfront fiber lease cost. In addition to 
%this, there are upfront equipment costs for lighting the fiber, and recurring maintenance costs, which is likely to 
%exceed the upfront costs for the entire lease term. Moreover, long-haul links require optical regeneration, which 
%requires maintaining and monitoring equipment in potentially difficult to reach places depending on the route. 

%Our analysis is here based on short term --means 3 to 5 years in this context-- wavelength leases. Depending on 

\begin{figure}
\centering
\includegraphics[width=3.2in]{figures/link_utils.pdf}
\caption{The CDFs of link utilization for different capacity links for the fiber network}
\label{fig:link-utils}
\end{figure}

Using an aggregate input rate of $1\text{Tbps}$, we computed the bandwidth needed per link for shortest-path routing.
For each link, we picked the wavelength capacity such that utilization would be $20$-$90\%$. For some links, this
meant using $2$ wavelengths of the same capacity.
%Based on required bandwidth and utilization constraints we used 2 wavelengths with the same capacity on some links. 
%Using our $\$ / (\text{Gbps} * \text{km})/\text{month}$ price estimates for different wavelength capacities we obtained 
%the cost for every link. 
Figure~\ref{fig:fiber-cost-stretch} shows
variation in cost with the number of network edges. Overall, cost is smaller with fewer edges, but as the network gets 
smaller, the increasing load on 
some links requires upgrading to higher capacity wavelengths, and as an artifact of this, we see 
higher costs for some networks with a small number of fewer edges. 

Based on a $5$ year lease, the cost of the network in figure~\ref{fig:fiber-design} is estimated to be 
$\$190$ million. This cost is dominated by bandwidth costs, which total to $\$168$ million over $5$ years; the rest being equipment and colocation cost.  
Amortized over the network's goodput over $5$ years, this cost estimate translates to $\$ 0.009 / \text{GB}$.
Even though this seems very low at first glance, it is about $10\times$ more expensive than that for the New York to 
Chicago $100\text{Gbps}$ link at $\$30,000$/month. However the total aggregate capacity of all links in the designed 
network is $14.4\text{Tbps}$ and average hop count is $9$, which roughly explains how we lose a factor of $10$.
As provisioned, the network has significant spare capacity on many links. Figure~\ref{fig:link-utils} 
shows the CDFs of utilization across links grouped by different capacity wavelengths. The highest utilization is observed between 
New York and Philadelphia, which then splits into heavy traffic routes towards Chicago and Washington D.C. 
This, of course, depends on the traffic model. We believe the cost estimates would not change dramatically under different traffic models
than the gravity model we use. A detailed analysis along these lines is omitted here, but included for the microwave-based network in the following.
%Our cost analysis here is coarse, but we believe it is representative for a ballpark estimate. 


==> proposal.tex <==
\section{Fast-Forward to the Future}
\label{sec:proposal}

In line with the community's understanding, our measurements affirm that TCP transfer and DNS resolution are important factors causing latency inflation. However, building a speed-of-light Internet requires addressing not only inflation due to protocols, but also that stemming from the Internet's infrastructure. Is this then, a lost cause, as infrastructural problems often are deemed to be? No! In fact, we present here a surprisingly low-cost solution to the infrastructural problem.
%, and argue that contrary to intuition, it might even be easier to address than the protocol factors.
\subsection{A parallel low-latency infrastructure} 
\label{subsec:microwave}

The approach we propose is to build a ``parallel Internet'' to move a select latency-sensitive portion of traffic along nearly the shortest paths on the Earth's surface at nearly the speed of light in vacuum.  

How might we build such a supplemental Internet infrastructure? In addressing this question, we draw inspiration from the industry which almost certainly places the highest premium on latency today: the high frequency trading (HFT) industry, which has already demonstrated the plausibility of operating long-distance links at nearly the speed of light in vacuum. The extraordinary value of possessing the fastest possible information transfer between financial exchanges in the New York and Chicago areas has led to steady and significant investment in low-latency infrastructure. In the mid-$1980$s, the round-trip latency was $14.5$ms. This was cut to $13.1$ms by $2010$ by shortening the physical fiber route.  Since then, value of low latency -- even in the presence of relatively lower bandwidth and reliability -- has led to the development of a number of competing microwave communication networks, which have cut the round-trip travel time to 
 $7.682$ ms\footnote{McKay Brothers, LLC; quoted latency for the CME Data Center, Aurora, IL  $\leftrightarrow$ NASDAQ Data Center, Carteret, NJ, \url{http://www.mckay-brothers.com/product-page/\#us}}, and see Fig.~\ref{fig:latencyImprovement}. The round-trip travel time between the same two locations along the shortest path on the Earth's surface at the speed of light in vacuum, is only $\sim0.1\,$ms less. A similar race is underway along multiple segments in Europe, including London-Frankfurt~\cite{microwaveEurope}, and a query of the FCC license database indicates that a transcontinental route linking Chicago to Seattle, in order to access NTT's PC-1 transpacific cable landing, is currently under construction.
 
 \begin{figure}
\centering
\includegraphics[width=3.5in]{figures/latencyImprovement}
\vspace{-10pt}
\caption{\small \em Evolution of the lagged limit order book response for the SPY Exchange Traded Fund (recorded at Nasdaq's Carteret, NJ matching engine) to traded price changes in the CME's E-Mini S\&P 500 Near-Month Futures contract which trades in Aurora IL  [see Laughlin, Aguirre \& Grundfest 2014 for our methodology]. The speed of light travel time is 3.92 milliseconds from Aurora to Carteret.  The latency improvement from 2010 to 2011 is due to Spread Networks' purpose-built \$300M fiber, which cut more than a millisecond off of the then-fastest fiber, achieving a latency of 6.65ms. The drop from 2011 to 2015 is primarily due to the appearance, proliferation and performance improvements of line-of-sight microwave networks connecting the two trading venues. The 2015 response function was measured on Aug 21, a day with both extraordinarily high volume and high market volatility. The two vertical lines mark lags of 4ms and 7ms.
}
\label{fig:latencyImprovement}
\vspace{-8pt}
\end{figure}
 
\paragraphb{Properties of microwave communication:} Microwave transmission has several properties advantageous for low-latency applications:

\begin{enumerate}
\item Microwave propagation through air (rather than fiber) reduces transit time by a factor of the fiber index of refraction $n\sim 1.4-1.6$. \item Between antennas at the link ends, a microwave beam travels in a perfectly straight line; the if links can be well-aligned, the route between two endpoints can be very close to the minimal length ``great circle" path.  
\item For bitrates of $< 1\,$Gbps, the deployment cost per Mbps per km travelled by microwave is considerably lower than by fiber (see Fig.~\ref{fig:mwvfiber} and discussion below). 
\item The deployment time and complexity is considerably lower than fiber, and an extensive tower, licensing, and other infrastructure exists in the U.S. to support microwave communications, with several hundred thousand microwave links currently licensed in the FCC database.
\item A weakness of digital microwave radios as of $\sim 5$ years ago was that digital signal processing introduced to increase throughput and uptime also adds considerable per-hop equipment latency ranging from 50\,$\mu s$ up to several ms per $\sim 50\,$km hop, effectively increasing the transmission time by anywhere from $\sim 30$\% up hundreds of percent.  However, the high-frequency trading latency race has led to the development of dozens of new radio models with per-hop latency of as little as a few $\mu s$ per hop, adding negligibly to the overall network latency.\footnote{See, e.g., \url{http://www.cielonetworks.com/site/white-papers.html}.}
\end{enumerate}

\begin{figure}
\centering
\includegraphics[width=3.5in]{figures/mwf}
\vspace{-10pt}
\caption{\small \em Approximate deployment cost per Mbps per km for Microwave (MW), Millimeter wave (MMW), and rural or urban fiber builds.  The individual bars, e.g. in blue, correspond to running 1, 2, 3, etc. links in parallel; as signified by the dotted lines, this becomes impractical after a few parallel links.  The lines slope downward because bandwidth comes at a fixed cost per link or per km of fiber, until the conduit saturates and a parallel link must be built.  This plot does not convey that for distances $d< 50$\,km, the MW links are (roughly) fixed cost whereas the fiber scales per km.  The plot exhibits the significant cost saves (of order a factor of 10) in MW or MMW relative to fiber for a network bitrates below several Gbps.  It should be noted that such links also entail considerable savings in deployment time and complexity.
}
\label{fig:mwvfiber}
\vspace{-8pt}
\end{figure}

The basic properties of microwave (MW) communication networks, in relation to fiber, are summarized in Fig.~\ref{fig:mwvfiber}.  MW communication spans the radio spectrum from approx. $2-90$\,GHz.  Key regions include the 5 GHz unlicensed band, the 6, 11, and 18 GHz licensed bands, and 70-90 GHz ``light licensed" bands; the latter are often referred to as ``millimeter wave" (MMW).\footnote{See \url{https://www.gpo.gov/fdsys/pkg/CFR-2009-title47-vol5/pdf/CFR-2009-title47-vol5-part101.pdf} for official details governing U.S. MW and MMW communications.}  

The 6-18 GHz bands are broken into 20-50 MHz channels; a typical MW radio operates in a single channel, though some can aggregate several channels.  A 30-40\,MHz channel can sustain data rates of 150-200\,Mbps, depending on modulation system, error correction, etc.  MW communication is vulnerable to disruption by precipitation, atmospheric effects, self-interference (``multipath fading"), and pointing errors. These effects decrease the signal-to-noise of the MW beam and can be partially compensated for using error correction and simpler encoding scheme; thus there is generally some tradeoff between data rate and radio uptime.  Two or more radios can often be multiplexed into a single pair of antennas.  Thus depending upon the available frequency spectrum, path characteristics, and uptime needs, a pair of antennas can support a link of up to $\sim 600-800\,Mbps$, and multiple dishes could support data rates a few times higher.  Topographic and weather/uptime considerations constrain 6-11 GHz links to less than 50-75\,km, and 18\,GHz links to less than $\sim 30$\,km.  Licensed (6-18 GHz) bands require registration within an FCC-enforced system; unlicensed (5 GHz) links require no licensing but are vulnerable to interference from other devices sharing the same spectrum.

MMW communications operate over a wider frequency space ($\sim 20 GHz$) and have accordingly much large channel sizes.  MMW radios can carry between 1\,Gbps to as much as 5-10\,Gbps per point-to-point link even using small antennas.  MMW in the US operates under a semi-volunteer frequency coordinate scheme that provides some protection from interference; the simplicity of this scheme along with much smaller equipment makes MMW much less complex and costly to deploy.  However, MMW propagation is limited by precipitation to $\sim 5\,km$.\footnote{Free-space optics, using infrared lasers has capabilities and costs broadly comparable to MMW systems.} 

In Fig.~\ref{fig:mwvfiber} we compare a ``light" MW build (one radio pair, relatively small antennae), a ``heavy" MW build (several multiplex radios, larger antennae), a MMW build, and fiber communication.  Including tower identification and leasing, potential tower retrofitting, equipment costs, installation costs, frequency coordination and licensing, and other costs, a ``light" MW build can cost of order USD\$50-100,000, with a ``heavy" build (several radios multiplexed onto larger antennas) a factor of two or more higher.  A ``heavy" MMW build (using several lower-bandwidth radios or one more expensive but more cutting-edge radio) is probably comparable to a light MW build.  In comparison, fiber costs per km of deployment are much higher, [[add references]] but at high bitrates become more cost-effective on a cost per km per Mbps basis.

We propose to leverage the strengths and new developments in microwave radio into a nationwide ``$c$-network" connecting population centers via a network of microwave links that is optimized to created the lowest possible latency communications to the largest number of users.  Of course, fashioning a practical solution from this approach requires careful decisions about the extent of such infrastructure's geographical coverage,  its capacity and usage, and how it connects with the existing telecommunications infrastructure. In the following, we address these design decisions first in the abstract, and then with a case study of such a proposal limited to the US.

\paragraphb{Geographical coverage:} Building a ubiquitous speed-of-light Internet with today's technology is likely to be cost-prohibitive, as it would replicate much of the existing telecommunications infrastructure built up over decades at great expense. A more reasonable approach is to connect centers of dense population into a $c$-network, and rely on existing infrastructure to reach areas up to $\sim100$\,km. Using fiber over $100$\,km incurs an additional $\frac{1}{3}$ms of latency round-trip in comparison with $c$-connectivity. Thus, even if the physical paths in these final $\sim 100$\,km of geo-distance are somewhat circuitous, we can expect the total latency overhead to be limited to $2$-$3$ms for such an end-to-end connection.\footnote{Additional latency may easily arise from local ISP handling, the cell network for cell connectivity, etc.  Some of these will be circumventable by latency-sensitive users.} The goal should be to cover the large distances at nearly $c$. 

Obviously, some scenarios pose difficulties for such a deployment. Building trans-Atlantic or trans-pacific microwave connectivity, for example, would be unlikely to make sense for general use (although the HFT industry is already considering the possibility of using weather balloons or drones to overcome that challenge~\cite{transAtlantic}.)  More likely would be possible future technologies such as ``hollow fiber''~\cite{hollowfiber}, or a low-Earth-orbit satellite network such as those mentioned below.  In the meantime, connecting the $c$-network to cable landings would still remove considerable latency from inter-continental communications.

\paragraphb{Capacity and usage:} Matching the present Internet's bandwidth in a parallel speed-of-light infrastructure would be exorbitantly expensive. However, most traffic on the Internet is not latency sensitive. For example, video streaming, file sharing, and software downloads comprise an overwhelming fraction of the traffic on the Internet. Further, even most interactive Web traffic consists of small requests (few KB) which fetch responses larger by two to three orders of magnitude. While small responses may be accommodated over the $c$-network, larger responses could be sent over traditional connectivity. If protocol overheads were negligible, this would still achieve $\frac{c}{2}$-connectivity overall. Thus, targeting $1\%$ of the latency sensitive Web traffic's capacity needs would be a reasonable goal. 
[[tie this into other parts of the paper.]]
\footnote{Admittedly, some latency-sensitive applications we discuss in \S\ref{sec:nfs} (such as tele-immersion) depend on both high bandwidth and low latency. While our present proposal may be inadequate for such applications at scale due to limited bandwidth, it still serves other applications such as instant access. We consider this work a start in this direction.}
%Our $c$-infrastructure proposal should thus target a small fraction of today's Internet's bandwidth needs, limiting its use to latency sensitive applications alone.

In some sense, this infrastructure may be easier to make progress on than many protocol changes, which depend on consensus among several stakeholders. It also has a healthy incremental deployment potential. An ISP might start by selling a low-latency transit service to other ISPs on a few critical routes. It might also be possible to market directly to end-users by making use of tunneling in a manner suggested by a recent research proposal~\cite{onetunnel}, where a user sends their packets first to an IP address connected to the $c$-network, which tunnels them to the exit from the $c$-network which is nearest to the packets' final destination. \nnn{(In this sense, the $c$-network uses ``cold potato'' routing.)}

In the following section, we analyze the coverage, capacity, and cost of a nearly speed-of-light network across the contiguous United States.

\subsection{A $c$-ISP in the US}

\paragraphb{Geographical coverage:} We focus on connecting only the $200$ most populous metropolitan areas in the contiguous United States
%\footnote{In an innocuous instance of experimenter bias, Champaign-Urbana was included at the expense of Topeka, Kansas at the bottom of our list.} 
with each other over this infrastructure. Further, we coalesce suburbs and cities in close vicinity of each other (within $50$ kilometers), ending up with $120$ population centers. Based on population data for $2010$~\cite{populationData}, we calculate that $\sim$$258$ million people comprising $\sim$$85\%$ of the US population live within $100$ kilometers of these $120$ population centers. 

\paragraphb{Capacity and usage:} Cisco's forecast for ``Consumer Internet Traffic'' for $2015$ in North America\footnote{An equivalent number for the contiguous US was not available. We note that the US population is only two-thirds of that of North America, but continue to use Cisco's North America traffic estimate without any proportional adjustment as a conservative upper bound for our analysis.} is $\sim$$11$,$500$ PB per month, \ie $\sim$$4.5$TBps~\cite{ciscoForecast}. Cisco also estimates that $78.5\%$ of Global IP traffic is file sharing and video, the rest ($22.5\%$) being classified as ``Web / Data'' traffic\footnote{It is worth noting that traffic such as software downloads (except when over P2P software) is included in the this category, but is not latency sensitive.}. This leaves a ceiling of $1$\,TBps for interactive Web traffic, and our goal is to design a low-latency network overlay that can handle a substantial fraction of order $\sim15$\% of this traffic. Cisco's report also claims that Web traffic is ``spread evenly throughout the day" unlike video, which has a ``prime time'' in each geography. Thus, we target $\sim 150$GB per second as our $c$-ISP's capacity. 

A MW network is built up of ``links" between towers (or sometimes buildings) on which antennas are mounted.  These chains of the links can form a ``route" between endpoints, which in our case corresponds to our population centers.
While new towers can be constructed, we restrict ourselves to using towers in databases including the  FCC's ``Antenna Structure Registration" database~\cite{fccasr} and databases from American Towers, Crown Castle, and several other tower companies for which were were able to download data.  We then culled this rather large database to a high-value subset of 12,080 microwave towers, for which we have evaluated line-of-sight suitability among 550,939 individual tower pairs.  For these purposes we assume that the antennas may be mounted near the top of the towers.  

The achievable hop length (which determines the number of towers required by a network linking a city pair) is limited primarily by Earth's curvature, and secondarily by reliability considerations.  The curvature constraint arises because the microwave path must clear the Earth as well as obstructions of height $h_{\rm obs}$ by approximately one Fresnel-zone width $h_{\rm Fres}$, and the Earth's curved surface can be treated as a ``bulge" of height $h_{\rm Earth}$ that a straight-line path must clear.  At the midpoint of a hop of length $D$, we have
$$
h_{\rm Fres} \simeq 8.7\,m\left(D\over 1\,{\rm km}\right)^{1/2}\left({f\over 1\,{\rm GHz}}\right)^{-1/2}
$$
and
$$
h_{\rm Earth} \simeq {1\over 50}\,m\left({D\over 1\,{\rm km}}\right)^2K^{-1},
$$
where $K$ accounts for the gradient of the atmospheric refractive index, which effectively multiplies the Earth's radius by a factor $K$.  (For this and other standard equations in microwave engineering, see e.g., Ref.~\cite{Manning}.)  Assuming tower of height $h_{\rm tow} \lesssim 100\,m$, $f \approx 6\,$GHz, $K < 4/3$, and $h_{\rm obs} \gtrsim 10\,m$, the constraint that $h_{\rm tow} > h_{\rm Fres} + h_{\rm Earth} + h_{\rm obs}$ requires $D \lesssim 70\,$km over flat terrain.  Intervening terrain peaks and valleys can increase or decrease this number, and it is also limited by tower availability, but this is a fairly accurate estimate, as existing, well-planned microwave networks spanning the $\sim 1200$\,km between New York and Chicago data centers require $\gtrsim 20$ hops.

We have employed an intuitive heuristic to design a network that simultaneously attempts to (1) connect as many population centers as possible, with (2) path length inflations (``stretch") between city pairs that are as small as possible, using (3) as small a number of towers as possible, and (4) respecting maximum link bandwidths while simultaneously minimizing the number of links that carry only a small fraction of their traffic capacity.

Our network map is constructed as follows. (1) We first rank the $N(N-1)/2=$7,140 city pairs by the products of their populations as a proxy for Internet traffic along the connecting routes.\footnote{A more accurate weighting could account for economic activity, as will as the geographical distribution of major data centers.} The \#1 population product is obtained for the New York City -- Los Angeles (NYC-LAX) city pair.

(2) We next use Dijkstra's algorithm calculate the shortest viable line-of-sight path between NYC and LAX that satisfies the physical constraints on all of its links (as given above). This optimal path uses 70 line-of-sight hops to span the 3961km geodesic distance, and has a summed edge length that is 61.2 km longer than the minimal distance, for an inflation factor of $1.015\times$. Because NYC-LAX defines the maximum traffic between any two city pairs, the traffic on this route defines a fiducial maximum bandwidth. In keeping with real-world link capacities (in which multiple frequencies are employed), we assume that 750 Mbps is available as the 1-way bandwidth on each link, with a small fraction of links carrying up to twice this amount (which might be accomplished by multiple antenna sets, etc.)

(3) We next proceed through the process of finding the shortest routes between the remaining ranked pairs, keeping track of the summed traffic on each link, and ``retiring'' a link once it exceeds the NYC-LAX fiducial traffic. This allows modest $<2\times$ overloading on a small subset of links, as a link is retired only after its traffic exceeds the 750 Mbps threshold. To prevent endpoints from being overloaded, we adopt city origin towers that  are further from the city center as the closest-proximity towers are saturated.

After considering all city pairs, and given the national inventory of towers that we have chosen, we find that of order 1,000 low-traffic city pairs out of the total 7140 total pairs have no viable direct city-to-city route due to link saturation. In addition, the resulting network is badly unbalanced, in the sense that some links are underutilized by a factor of $\sim$1000 in comparison to the NYC-LAX links. (The population product of NYC-LAX is more than 1000$\times$ that of a small pair such as Waco-Amarillo).  We then:

(4) De-activate all links in the network that carry less than $x$=2\% of the NYC-LAX traffic. Re-run steps 2-3 using this restricted link set.

(5) Repeat step 4 for progressively larger fractions $x$, such that $x$=5,10,15,20,25,30,35,40\%. 

The goal of this heuristic is to drive traffic onto a relatively balanced configuration, by (via step 4) eliminating low-traffic links and forcing the corresponding routes onto other higher-traffic links, while (via step 2) preventing links from becoming over-saturated.

\begin{figure*}
\centering
\includegraphics[width=6in, angle=0]{figures/networkmap}
\vspace{-10pt}
\caption{\small \em This plot shows our example of a US-wide wireless latency-optimized network.  The network links 84 cities (open boxes) using 3,950 unique point-to-point line-of-sight microwave ($\sim$ 6-11 GHz) radio links, each between two existing towers taken from FCC and other databases.  The network represents 1,762 routes between city pairs, and the color and weight assigned to each link represents the summed network traffic from city-to-city routes using that link. }
\label{fig:networkmap}
\vspace{-8pt}
\end{figure*}

With the demand that links carry 40\% of the NYC-LAX traffic, we show the resulting network map in Fig.~\ref{fig:networkmap}. 
The network is very efficient.  The city pairs are  separated by an average $d=$1387 km, so individual routes between city pairs would run a total of 2.4M km.  The total length of all of the links is 226,536 km, a factor of ten less. (More efficiency, furthermore, could be attained using a less stringent cap on dynamic range.) The network has a very good distribution of stretch (latency divided by $c$-latency), as shown in Fig.~\ref{fig:proposal_stretch}.

\begin{figure}
\centering
\includegraphics[width=2.6in]{figures/proposal_stretch}
\vspace{-8pt}
\caption{\small \em The latency stretch histogram for the 1.762 city-to-city routes. [[ to be replaced]]}
\label{fig:proposal_stretch}
\end{figure}

[[add to below: some mention of the latency-uptime-bandwidth-cost tradeoffs]]

\paragraphb{Economics:} At a plausible cost of \$50K-\$100K/link, the total network deployment cost would be \$200M-\$400M; including 5-year operating costs would perhaps increase this figure by 50-100\%.  We believe this may well be a conservative estimate because major economies of scale could be realized in such a project, and unlike many telecommunications deployments there is significant flexibility in how exactly the routes are laid out so that highly congested areas, faulty towers, and other sources of difficulty can be at least somewhat avoided.

Under our assumption that the LA-NYC traffic corresponds to 750 Mbps duplex, the aggregate traffic over the network is 150 Gbps.  
This represents 150,000 Mbps/(8 b/B)$\times$(2.6$\times10^{6}$ s/mo) = 5$\times10^{10}$ MB/mo.  If the cost is $5\times10^{8}$/5 yrs = $8\times10^{6}$/mo, we find 6 GB/\$ over 5 years (after this time, the cost is even lower as only OpEx and upgrade costs must be included.)

By way of comparison, the Internet2 predecessor, Abilene, cost \$$735$ million ($1998$ adjusted to 2017)~\cite{abileneCost}. That other ambitious projects with substantially larger price-tags are making progress is also encouraging; among these are OneWeb's plan to expand the reach of the Internet using a total of $648$ satellites in low-Earth orbit at an estimated cost of \$$1.5$-$2$ billion~\cite{arsGlobalInternet}, and a broadly similar effort from WorldVu, cost estimates for which range from \$$10$ billion to $15$ billion~\cite{arsGlobalInternet, muskTelegraph}.  (Note that these all these estimates are based on significant advances in the cost-effectiveness of satellite launches.)
Arctic Fiber is spending \$$850$ million to build a submarine cable through the Arctic, focused primarily on shortening the London-Tokyo route~\cite{arcticCable}.

Obviously, our analysis here is coarse, with many opportunities for refinement of the network's design. (For example, we combining microwave, millimeter wave, and fiber -- all with rather different characteristics -- could provide an even more efficient network.) However, the larger point is that a nearly speed-of-light infrastructure is feasible to build today relatively cheaply using well-proven technology.


\subsection{A one RTT transaction protocol}
\label{subsec:protocols}

As we note in \S\ref{sec:whyslow}, while eliminating infrastructural latency inflation will speed up the Internet by more than $3\times$, without any progress on transport protocols, this may still leave us more than $10\times$ away from $c$-latency in the typical case. Thus, while the main contributions of this work are our measurements and analysis highlighting latency inflation due to infrastructural inefficiencies, and our proposal for a nearly speed-of-light physical infrastructure, we also discuss here the possibility of building a one RTT transaction protocol for the Internet by putting together various protocol advancements the community's research has produced.

\paragraphb{DNS:} One possibility to speed up DNS lookups is simply brute replication of DNS infrastructure. Along the lines we argued in \S\ref{sec:nfs}, the $c$-infrastructure helps reduce the number of replicas needed to achieve a latency bound -- for example, within the contiguous US, just $7$ replicas would be enough to serve most of the population within $5$ms. \cut{Further, given our observations about the impact of tail DNS latencies, work that suggests making multiple redundant DNS queries from different DNS providers and using the fastest result~\cite{vulimiri} seems promising.} An alternate approach is to try achieving `on-path' lookups in a manner proposed by ASAP~\cite{asap}, where the client sends its data request itself to the DNS server, which resolves the destination's address and forwards the data request on behalf of the client. Another method of achieving `on-path' lookups is name-based routing. However these latter methods have their limitations, requiring extensive architectural changes.

\paragraphb{Eliminating the TCP handshake:} In the absence of a handshake, a malicious client may craft packets with a source address different from its own, thus causing the server to send the response to that address. This technique can be used to attack both the server and other end hosts (which may receive large volumes of data from several servers directed to them by malicious clients). The handshake, by requiring that the client acknowledge a message with a nonce before any significant compute or network resources are spent by the server, prevents this. Avoiding the handshake thus entails address authentication by some other means. Several solutions are available, including ASAP~\cite{asap}, TCP Fast Open's Cookie mechanism~\cite{fastopen}, and APIP~\cite{apip}, with the broad idea being that the server (or another accountable third-party) validates the client's claim to the address (or, in APIP's case, the data packets); subsequently, this validation is included with future requests thus eliminating the handshake for those requests. The latency cost of validation may be incurred much less frequently than with handshaking for each connection.

\paragraphb{Eliminating TCP slow-start:} As we see in \S\ref{sec:whyslow}, TCP's slow start mechanism implies that fetching even just a few tens of kilobytes requires several RTTs. A variety of possibilities exist for handing this problem, the simplest proposal being to use larger TCP initial window sizes~\cite{dukkipati}. In our scenario, one could consider sending a larger TCP window's worth of data over the $c$-infrastructure, and another few tens of kilobytes (if necessary) across traditional connectivity. There are of course, other options, such as Jumpstart~\cite{jumpstart}, which allows for any `appropriate' rate from the beginning, where the appropriate rate may be determined in several possible ways; for example, ISPs could maintain a per-prefix listing of suitable window sizes based on recent history, etc. Another proposal addressing the slow-start problem, RC$3$~\cite{rc3} suggests using multiple priority levels, sending out a small volume at the highest priority, and an exponentially increasing volume of data at successively lower priority levels, thus sending out a large volume of data right from the start, while removing the possibility of congestion collapse. (In RC$3$, packets at each priority obey TCP's congestion collapse directives.) RC$3$ does however pose deployment hurdles, requiring that all routers support multiple priorities.

\paragraphb{TLS/SSL:} In addition to the various protocol pieces above, making \emph{secure} connections quickly is also an important problem. Google's experimental QUIC protocol~\cite{quic} may present a solution here. QUIC proposes that once a client has a server's public key (perhaps through a prior contact, which does require an additional round-trip), it can send its data request, together with a proposed session key, all encrypted with the server's public key. The server can accept the session key (in the common case) and encrypt the response with it. Of course, QUIC too requires the elimination of the handshake and slow-start, and how exactly each objective will be met is currently being worked out. 
%We believe that obtaining the server's public key can be rolled into the DNS resolution step, where the DNS server responds to the client with both the IP address and public key of the server.

QUIC's modular design makes it a useful vehicle for protocol improvements such as eliminating the TCP handshake and folding in a more aggressive congestion control algorithm. Encouragingly, Google's servers already support it, and while it is at this stage experimental, with several pieces of the design yet to be frozen, clients using Google's Chrome browser or Opera can enable it~\cite{quic}.

\nnn{The $c$-network could also spur the development and use of new protocols, for instance, by using new protocols internally and deploying proxies at the edge. This would be similar to what Akamai's SureRoute~\cite{sureRoute} does (in terms of maintaining persistent TCP connections between Akamai servers.)}

